Background Splitting: Finding Rare Classes in a Sea of Background

We focus on the real-world problem of training accurate deep models for image classification of a small number of rare categories. In these scenarios, almost all images belong to the background category in the dataset (>95% of the dataset is background). We demonstrate that both standard fine-tuning approaches and state-of-the-art approaches for training on imbalanced datasets do not produce accurate deep models in the presence of this extreme imbalance. Our key observation is that the extreme imbalance due to the background category can be drastically reduced by leveraging visual knowledge from an existing pre-trained model. Specifically, the background category is "split" into smaller and more coherent pseudo-categories during training using a pre-trained model. We incorporate background splitting into an image classification model by adding an auxiliary loss that learns to mimic the predictions of the existing, pre-trained image classification model. Note that this process is automatic and requires no additional manual labels. The auxiliary loss regularizes the feature representation of the shared network trunk by requiring it to discriminate between previously homogeneous background instances and reduces overfitting to the small number of rare category positives. We also show that BG splitting can be combined with other background imbalance methods to further improve performance. We evaluate our method on a modified version of the iNaturalist dataset where only a small subset of rare category labels are available during training (all other images are labeled as background). By jointly learning to recognize ImageNet categories and selected iNaturalist categories, our approach yields performance that is 42.3 mAP points higher than a fine-tuning baseline when 99.98% of the data is background, and 8.3 mAP points higher than SotA baselines when 98.30% of the data is background.

==> acks.tex <==
\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare 
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

==> problem.tex <==
\section{Problem Setup}
\label{sec:problem}

\bill{We have agreed to delete this section, moving any non-redundant info to the intro, related work, or evaluation sections}

Imbalanced, long-tail datasets like iNaturalist \cite{gvanhorn2018inat} are composed of a long-tail of rare categories and are densely annotated with positives--every image is annotated with at least one instance of a category. 
We consider the setting in which the focus is on the accuracy of a model in classifying a specific set of rare categories, rather than an entire long-tailed distribution of categories which can be more costly to annotate. When only annotating for a target set of rare categories, the vast majority of examples in an imbalanced, long-tailed dataset will not contain any positive instances of those categories. 

To simulate the practical setting we are interested in, we select a random set of rare categories, the \emph{foreground} categories, from the total set of 5089 categories.  We construct the sparse positive dataset by mapping all the labels for all other categories not included in the foreground categories to the background category.


While we focus on the performance of models on the set of $N$ rare categories, we also investigate how including labels from other categories in the dataset affects the performance of the final model. We denote the entire number of included categories and their labels as $M$, which includes the $N$ rare categories. \kf{notation.  Intro has $M$, here there is a $K$.}
\deva{updated notation. my suggestion is to follow the intro and methods. We are training "$N+1$-way classifiers on the full iNaturalist training set, and evaluate them on Sparse iNaturalist."}
